Chern Numbers of Matroids

We define Chern numbers of a matroid. These numbers are obtained when intersecting appropriate matroid Chern-Schwartz-MacPherson cycles defined by L\'opez de Medrano, Rinc\'on, and Shaw. We prove that when a matroid arises from a complex hyperplane arrangement the Chern numbers of the matroid correspond to the Chern numbers of the log cotangent bundle. A matroid of rank 3 has two Chern numbers. We prove that they are positive and that their ratio is bounded by 3, which is analogous to the Bogomolov-Miyaoka-Yau inequality. If the matroid is orientable, we generalize a result of Eterovi\'c, Figuera, and Urz\'ua to prove that the ratio is bounded above by 5/2. Finally, we give a formula for the Chern numbers of the uniform matroid of any rank.

==> Introduction.tex <==
\section{Introduction}
\label{sec:intro}
Matroids are combinatorial objects that abstract the notion of independence throughout several branches of mathematics. The Japanese mathematician Takeo Nakasawa and the American mathematician Hassler Whitney independently developed the theory of matroids in the 1930s. \\ 
 \\
Our take on matroid theory will be from an algebraic geometry perspective. More specifically, given a hyperplane arrangement $\mathcal{A}\subseteq \mathbb{P}^{d+1}_k$, there is an associated matroid $M_\mathcal{A}$ which encodes the combinatorial properties of the linear subspaces of $\mathcal{A}$. 
Matroids that are constructed in this way are called \textit{representable over a field} $k$. A matroid is \textit{representable} if it is representable over any field. Note that representable matroids constitute about $0\%$ of all matroids \cite{nelson2016almost}.
A natural question is: can we define invariants of a general matroid, i.e., a matroid that is not necessarily representable, which have a geometric meaning when the matroid is in fact representable? \\
\\
We introduce a new invariant of matroids, namely the \textit{Chern numbers} of a matroid, which are numbers obtained when intersecting \textit{Chern Schwartz MacPherson cycles} (CSM cycles) of matroids, certain weighted polyhedral fans that are given by the matroid. \\ 
 \\ 
More specifically, to a matroid $M$ of rank $d+1$ we can assign a rational polyhedral fan $\Sigma_M$ called the \textit{Bergman fan} of $M$ (\cref{def: Bergman}) having a cone for each chain of flats of $M$ introduced by Ardila. %To the Bergman fan $\Sigma_M$ of a matroid $M$ we can consider the \textit{Minkowski weights} $MW_k(\Sigma_M)$ supported on $\Sigma_M$. 
The additive group of $k$-dimensional \textit{Minkowski weights} $MW_k(\Sigma_M)$ consist of the the weighted $k-$skeletons of the fan $\Sigma_M$ satisfying the balancing condition. Minkowski weights were first studied in the more general context of complete toric varieties in \cite{fulton1997intersection}. Minkowski weights have a ring structure given by a certain intersection product that can be defined in several ways. For example, Shaw gives a recursive definition based on tropical modifications and contractions \cite{shaw2013tropical}. While Fran{\c{c}}ois and Rau construct an intersection product via intersecting with the diagonal \cite{franccois2013diagonal}. Moreover there exists an isomorphism $w: MW_0(\Sigma_M)\rightarrow \mathbb{Z}$, naturally defined by the weight assigned to the vertex of the fan.\\ 
 \\
L\'opez de Medrano, Rinc\'on, and Shaw introduce in \cite{de2020chern} the \textit{Chern-Schwartz-MacPherson (CSM) cycles} of a matroid. The weights of the $k$-dimensional CSM cycle $\text{csm}_k(M)\in MW_k(M)$ are determined by the characteristic polynomial of matroid minors. The authors prove that the CSM cycles of a matroid are related to the CSM classes in algebraic geometry. These classes are a generalization of the Chern class of the tangent bundle over a non-singular compact variety. When the matroid $M_\mathcal{A}$ arises from an arrangement $\mathcal{A}$, the authors prove that 
$$\text{CSM}(1_{C(\mathcal{A})})=\sum_{k=0}^d \text{csm}_k(M_\mathcal{A})\in MW_*(\Sigma_{M_\mathcal{A}}),$$
where $\text{CSM}(1_{C(\mathcal{A})})$ is the CSM class of the group of constructible function on the complement of the arrangement $C(\mathcal{A})$. \\ 
\\
In the more general context of algebraic geometry, the \textit{Chow ring} of a variety is a ring generated by the cycles of the variety, quotient by rational equivalence. For matroid $M$, the Chow ring $A^*(M)$ is a polynomial ring given by 
\begin{align*}
    A^*(M)=\frac{\mathbb{Z}[x_F:\ F \text{ is a flat of }M]}{\mathcal{I}_M+\mathcal{J}_M}, 
\end{align*}
where $\mathcal{I}_M$, and  $\mathcal{J}_M$ are ideals encoding the inclusion properties of the flats introduced by Feichter and Yuzvinsky in \cite{feichtner2004chow}. The authors proved that when the matroid arises from a hyperplane arrangement, then the Chow ring of the matroid is isomorphic to the Chow ring of the de Concini and Procesi \textit{wonderful compactification of the complement of the arrangement} $W_\mathcal{A}$ \cite{de1995wonderful}. 
Moreover, Adiprasito, Huh, and Katz proved that the Chow ring of a matroid satisfies Poincar\'e duality and linear duality \cite{adiprasito2018hodge}, which give us the following isomorphism
\begin{equation}
\label{eq: 1}
    A^*(M)\cong MW_*(\Sigma_M).
\end{equation}
Note that besides from a few special cases, computing the intersection product of Minkowski weights can be quite hard. However, by the isomorphism given in \cref{eq: 1}, we can assign to every k-dimensional Minkowski weight a unique degree $(d-k)$-polynomial in the Chow ring. Rinc\'on and Fife have found an explicit formula for representing the CSM cycles of the Bergman fan of the matroid in the Chow ring\todo{Ask for a reference}. Hence, when intersecting CSM cycles we can simply multiply the corresponding polynomials in the Chow ring. \\ 
 \\
We define Chern numbers of a matroid to be multiplicities associated to the vertex of the fan when intersecting appropriate CSM cycles of a fixed matroid, in order to get a zero dimensional intersection.
\begin{comment}  
A \textit{k-dimensional Minkowski weight} is obtained by assigning weights on the $k$-skeleta of the fan $\Sigma_M$ satisfying the balancing condition. 
\end{comment}



\begin{definition}(Definition \ref{def: c numbers})
Let $M$ be a rank $d+1$ matroid. We define the \textit{Chern numbers of a matroid} $\bar{c}_1^{k_1}\bar{c}_2^{k_2}\cdots \bar{c}_d^{k_d}(M)$ to be
$$\bar{c}_1^{k_1}\cdots \bar{c}_d^{k_d}(M)= \text{w}(\text{csm}_{d-1}^{k_1}(M)\text{csm}_{d-2}^{k_2}(M)\cdots \text{csm}_0^{k_d}(M)),$$  where $\sum_{i=0}^d i\cdot k_i=d$, and the map $\text{w}$ is the map returning the multiplicity associated to the vertex.
\end{definition} 
The inspiration for studying these numbers comes from results in the study of geography of manifolds which deals with the possible values of Chern numbers of algebraic manifolds of general type, see for example  \cite{hunt1989complex}. In fact, our main result relates Chern numbers of matroids to Chern numbers of algebraic manifolds.
\begin{thm}
Let $\mathcal{A}\subset \mathbb{P}^n_\mathbb{C}$ be a hyperplane arrangement and let $M_\mathcal{A}$ be the corresponding matroid. Let $W_\mathcal{A}$ be the maximal wonderful compactification of its complement $C(\mathcal{A})$ and let $D= W_\mathcal{A} \setminus C(\mathcal{A})$. Let $\Omega^1_{W_\mathcal{A}}(\text{log}\ D)$ denote the bundle of log differentials on $W_\mathcal{A}$ with poles along $D$ and $\Omega^1_{W_\mathcal{A}}(\text{log}\ D)^*$ denote its dual. Then 
$$\bar{c}_1^{k_1}\cdots \bar{c}_d^{k_d}(\Omega^1_{W_\mathcal{A}}(\text{log} D)^*)=\bar{c}_1^{k_1}\cdots \bar{c}_d^{k_d}(M_\mathcal{A}).$$
\end{thm} 
In \cref{prop: Chern3} we prove that there is an explicit formula for Chern numbers of simple matroids of rank 3 in terms of the flats. Note that when a matroid is representable over some field $k$, it arises from a line arrangement over $k$. In fact our formula corresponds to Eterovi\'c, Figuera and Urz\'ua definition for the Chern numbers of line arrangements. In the rest of \cref{sec: ch3} we prove results concerning bounds on the Chern numbers of simple matroids of rank 3.

\begin{proposition}
\cref{prop: new bounds}
Let $M$ be a simple matroid of rank $3$ on a ground set $E$ of size $n+1$. The Chern numbers $\overline{c}_1^2(M)$ and $\overline{c}_2(M)$ are bounded by
\begin{align*}
     0\leq \overline{c}_1^2(M)&\leq \overline{c}_1^2(U_{3,n}),\ \textup{and} \\
    0\leq \overline{c}_2(M)&\leq\overline{c}_2(U_{3,n}).
\end{align*}
\end{proposition}

\begin{thm}
\cref{thm: bounds ch 3}
Let $M$ be a simple matroid of rank $3$ on $E=\{1,\ldots,n\}$ with no coloops. Then,
\begin{align*}
    \frac{2n-6}{n-2}\leq \frac{\overline{c}_1^2(M)}{\overline{c}_2(M)}\leq 3.
\end{align*}
Left equality holds if and only if M is the uniform matroid $U_{3,n}$, and right equality holds if and only if M is the matroid of a finite projective plane.
\end{thm}
The right inequality, is in fact the same inequality for the quotient of the Chern numbers of complex algebraic surfaces given some restrictions, which is known as the \textit{Bogomolov-Miyaoka-Yau inequality}. 
The next theorem is a generalization of a result due to Hirzebruch when considering line arrangements \cite{hirzebruch1983arrangements}.
\begin{thm}\ref{thm: orientable}
If $M$ is a simple orientable matroid of rank 3 with no coloops, then 
\begin{align*}
    \frac{\overline{c}_1^2(M)}{\overline{c}_2(M)}\leq \frac{5}{2}.
\end{align*}
 Equality is achieved if and only if the pseudoline arrangements of M are simplicial.
\end{thm}
To further motivate the study of Chern numbers of matroids we pose the following questions. 
\begin{ques}[Geography of Chern number pairs in rank 3]
\label{question: range}
For which pairs $(a,b)\in \mathbb{Z}_{\geq 0}\times \mathbb{Z}_{\geq 0}$ does there exists a matroid such that $$(\overline{c}_1^2(M), \overline{c}_2(M))=(a,b)?$$ 
\end{ques}
Question \cref{question: range} is related to the study of the geography of Chern numbers of surfaces in complex algebraic geometry, where more about these numbers is known, see for example \cite{EncyMath} for a brief overview, or \cite{hunt1989complex}. 
\begin{ques}[Representability of Chern numbers in rank 3]
\label{question: realizability 3}
Given any simple matroid $M$ of rank 3 with Chern numbers $(\overline{c}_1^2(M),\overline{c}_2(M))$, does there exist a representable matroid $M_\mathcal{A}$ over some field $k$ of rank $3$ such that $$(\overline{c}_1^2(M_\mathcal{A}), \overline{c}_2(M_\mathcal{A}))=(\overline{c}_1^2(M), \overline{c}_2(M))?$$ 
\end{ques}
Finally, we want to point out the possible extent of these questions. Recall, from \cref{thm: bounds ch 3}, that for a simple matroid of rank 3 the quotient $\overline{c}_1^2(M)/\overline{c}_2(M)=3$ if and only if $M$ is the matroid of a finite projective plane. Moreover, in \cref{ex: ch PG(2 q)} we show that the finite projective plane matroid $PG(2,q)$ of order $q$ has Chern numbers 
\begin{align*}
  \overline{c}_1^2(PG(2,q))=&3(q^3-q^2-q+1),\\
    \overline{c}_2(PG(2,q))=&q^3-q^2-q+1.
\end{align*}
Hence, finding out for which values of $q$ there exists a matroid $M$ having Chern numbers $(\overline{c}_1^2(M),\overline{c}_2(M))=(3(q^3-q^2-q+1),q^3-q^2-q+1)$, and if so if the matroid is representable over a field, would in fact solve the prime power conjecture.  

\begin{comment}
\begin{proposition}
\label{prop: ch positive}
Let M be a simple matroid of rank $3$ on the ground set $E = \{1,\ldots,n\}$, and let $t_m$ be the number of flats of rank $2$ of size $m$. If M has no coloops then its Chern numbers are positive.
\end{proposition}
\begin{proposition}
\label{prop: new bounds}
Let $M$ be a simple matroid of rank $3$ on a ground set $E$ of size $n+1$. If $M$ has no coloops, then the Chern numbers $\overline{c}_1^2(M)$ and $\overline{c}_2(M)$ are bounded by
\begin{align*}
     \overline{c}_1^2(M)&\leq \overline{c}_1^2(U_{3,n+1}),\ \textup{and} \\
    \overline{c}_2(M)&\leq\overline{c}_2(U_{3,n+1}).
\end{align*}
\end{proposition}
\begin{thm}
\label{thm: bounds ch 3}
Let $M$ be a simple matroid of rank $3$ on $E=\{1,\ldots,n\}$ with no coloops. Then,
\begin{align*}
    \frac{2n-6}{n-2}\leq \frac{\overline{c}_1^2(M)}{\overline{c}_2(M)}\leq 3
\end{align*}
Left equality holds if and only if M is the uniform matroid $U_{3,n}$, and right equality holds if and only if M is the matroid of a finite projective plane.
\end{thm}
\end{comment}

\begin{comment}
The \textit{Chow ring} of a variety is a ring generated by the cycles of that variety, quotient by rational equivalence. For matroid $M$, the Chow ring $A^*(M)$ is a polynomial ring given by 
\begin{align*}
    A^*(M)=\frac{\mathbb{Z}[x_F:\ F \text{ is a flat of }M]}{\mathcal{I}_M+\mathcal{J}_M}, 
\end{align*}
%where $\mathcal{I}_M$ is an ideal generated by quadric monomials corresponding to non-comparable flats, and $\mathcal{J}_M$ is an ideal generated by linear polynomials encoding the inclusion properties of the flats.
where $\mathcal{I}_M$, and  $\mathcal{J}_M$ are ideals encoding the inclusion properties of the flats. The Chow ring of a matroid has some important properties. First of all, Feichter and Yuzvinsky proved in \cite{feichtner2004chow} that when the matroid arises from a hyperplane arrangement, then the Chow ring the matroid is isomorphic to the Chow ring of the de Concini and Procesi \textit{wonderful compactification of the complement of the arrangement} $W_\mathcal{A}$ \cite{de1995wonderful}.

BLABLA 

Finally, we want to emphasise some of the extent of the study of Chern numbers of matroids. 
L\'opez de Medrano, Rinc\'on, and Shaw introduce in \cite{de2020chern} the \textit{Chern-Schwartz-MacPherson (CSM) cycles} of a matroid. The weights of the $k$-dimensional CSM cycle $\text{csm}_k(M)\in MW_k(M)$ are determined by the characteristic polynomial of matroid minors. The authors prove that the CSM cycles of a matroid are related to the CSM classes in algebraic geometry. These classes are a generalization of the Chern class of the tangent bundle over a non-singular compact variety. When the matroid $M_\mathcal{A}$ arises from an arrangement $\mathcal{A}$, the authors prove that 
L\'opez de Medrano, Rinc\'on, and Shaw introduce in \cite{de2020chern} the \textit{Chern-Schwartz-MacPherson (CSM) cycles} of a matroid. The weights of the $k$-dimensional CSM cycle $\text{csm}_k(M)\in MW_k(M)$ are determined by the characteristic polynomial of matroid minors. The authors prove that the CSM cycles of a matroid are related to the CSM classes in algebraic geometry. These classes are a generalization of the Chern class of the tangent bundle over a non-singular compact variety. When the matroid $M_\mathcal{A}$ arises from an arrangement $\mathcal{A}$, the authors prove that 
\end{comment}
\todo[inline]{Consider including the volume polynomial of Chris Eur}

==> figures/pappus.tex <==
%pappus
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]
\draw [line width=1pt] (-1.72,3.99)-- (2,0);
\draw [line width=1pt] (-1.72,3.99)-- (0,0);
\draw [line width=1pt] (0.72,3.99)-- (-2,0);
\draw [line width=1pt] (0.72,3.99)-- (2,0);
\draw [line width=1pt] (2.74,4.05)-- (0,0);
\draw [line width=1pt] (2.74,4.05)-- (-2,0);
\draw [line width=1pt] (-2.3,4.006843575418994)-- (3,4.0586592178770955);
\draw [line width=1pt] (-2.3,0)-- (3,0);
\draw [line width=1pt] (-2.3,1.6425)-- (3,2.1952095808383234);
\begin{scriptsize}

%\node at (-2,-0.5) {\Huge 4};
\draw [fill=black] (-2,0) circle (2pt);
\draw [fill=black] (0,0) circle (2pt);
\draw [fill=black] (2,0) circle (2pt);
\draw [fill=black] (-1.72,3.99) circle (2pt);
\draw [fill=black] (0.72,3.99) circle (2pt);
\draw [fill=black] (2.74,4.05) circle (2pt);
\draw [fill=black] (-0.7747747747747746,1.7972972972972974) circle (2pt);
\draw [fill=black] (1.3512000348467468,2.022431141376156) circle (2pt);
\draw [fill=black] (0.2233103065014888,1.905642977704049) circle (2pt);
\end{scriptsize}
\end{tikzpicture}

